BECoTTA: Input-dependent Online Blending of Experts for Continual Test-time Adaptation

Continual Test Time Adaptation (CTTA) is required to adapt efficiently to continuous unseen domains while retaining previously learned knowledge. However, despite the progress of CTTA, it is still challenging to deploy the model with improved forgetting-adaptation trade-offs and efficiency. In addition, current CTTA scenarios assume only the disjoint situation, even though real-world domains are seamlessly changed. To address these challenges, this paper proposes BECoTTA, an input-dependent and efficient modular framework for CTTA. We propose Mixture-of Domain Low-rank Experts (MoDE) that contains two core components: (i) Domain-Adaptive Routing, which helps to selectively capture the domain adaptive knowledge with multiple domain routers, and (ii) Domain-Expert Synergy Loss to maximize the dependency between each domain and expert. We validate that our method outperforms multiple CTTA scenarios, including disjoint and gradual domain shits, while only requiring ~98% fewer trainable parameters. We also provide analyses of our method, including the construction of experts, the effect of domain-adaptive experts, and visualizations.

==> dummy/04_prelim.tex <==
% \section{Preliminaries}

% \subsection{Problem Statement}    
% Continual Test-time Adaptation (CTTA) strives to adapt the source model $\bm{\theta_s}$ to continuously changing target domains $\bm{X^t}=\{X_1^t, X_2^t, .. X_c^t\}$. 
% In CTTA, a specific set of $C$ target domains is repeated in a pre-defined order for $M$ rounds to evaluate the long-term adaptation process. 
% Therefore, the primary goal of CTTA is to adapt to each target domain at each timestep without forgetting $\bm{\theta_s}$. 
% For each target domain sample $\bm{x^t_c}$, the segmentation model $\bm{\theta_c}$ from the current target domain $c$ predicts the logits of output prediction $\hat{y_c}$. 
% With $\hat{y_c}$ for each sample and its confidence value, we need to accurately predict the pixel-wise class labels without severely forgetting the knowledge of $\bm{\theta_s}$. 
% In this manner, the performance is commonly evaluated by iterating $N$ target domains for $M$ rounds. 
 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Mixture of Adapters (MoA)}     

% For the efficient CTTA, we adopt Mixture-of-Adapters (MoA) that constructs experts as adapters, which is inspired by the Sparse Mixture-of-Experts (SMoE). 
% For the routing policy, we mainly utilize top-k routing~\cite{moe1}.
% Each MoA layer consists of router $G$ and a set of $N$ lightweight adapters (i.e., experts), $A_1$, $A_2$, ..., $A_N$. 
% The former is parameterized by $\bm{W}_g$ and $\bm{W}_{noise}$, and the latter consists of two feed-forward networks and an activation function, $\bm{W}^{down}$,$\bm{W}^{up}$, and $\sigma(\cdot)$, respectively. 
% If the $A_i$ is activated, it maps the input $\bm{x}$ into the low dimensional space by projection operation with $\bm{W_i}^{down}$. And, after regularizing the features with a non-linear activation function $\sigma$, it recovers the features to the original dimension using $\bm{W_i}^{up}$. 


==> dummy/05_methods_v1.tex <==
\section{Methodology} 
\begin{figure*}[h]
    \centering
    {\includegraphics[width=0.85\textwidth]{./fig_v2/main_v3.pdf}}
    \caption{\textbf{Our main architectures.} We propose BECoTTA which addresses dynamic real-world continual scenarios including disjoint and gradual shifts. Our MoDLoRA layers ensure efficient input-dependent domain knowledge transfer while continual adaptation. The gray parts in the figure represent the frozen parts while conducting CTTA.}
    \label{fig:tent}
    \vspace{-0.5cm}
\end{figure*}

Our main goal was to guarantee the \textbf{\textit{domain-wise}} and \textbf{\textit{input-dependent}} process which deal with dynamic continual TTA scenarios (disjoint or gradual) while considering efficiency. 
To achieve this, we mainly propose a Mixture of Domain Low-Rank Adapters (MoDLoRA) architecture with mutual information loss to sparsely update domain-wise knowledge.

\subsection{Problem Statements}    
% v2 - from supple
% Test-Time Adaptation (TTA) aims to adapt to a static target domain without the source domain dataset $\bm{X_s}$. 
% In contrast, 
Continual Test-time Adaptation (CTTA) strives to adapt the source model $\bm{\theta_s}$ to continuously changing target domains $\bm{X_t}=\{X_{t1}, X_{t2}, .. X_{tN}\}$. 
In CTTA, a specific set of $N$ target domains is repeated in a pre-defined order for $M$ rounds to evaluate the long-term adaptation process. 
Therefore, the primary goal of CTTA is to adapt to each target domain at each timestep without forgetting $\bm{\theta_s}$. 
For each target domain sample $\bm{x_t}$, the segmentation model $\bm{\theta_t}$ which is adapted to the current target domain $t$ predicts the logits of output prediction $\hat{y_t}$. 
With $\hat{y_t}$ for each sample and its confidence value, we need to accurately predict the pixel-wise class labels without severely forgetting the knowledge of $\bm{\theta_s}$. 
% In this manner, the performance is commonly evaluated by iterating $N$ target domains for $M$ rounds. 

\subsection{Domain-wise Preprocessing}        % tentative title  
To ensure the domain-specific decision in the CTTA process, we conducted preprocessing before deploying continual scenarios. 

\textbf{Predefined domains.}     
We first set the probable domains for the warm-up process.
For pre-defining $D$ domains, we mainly focus on the variations in the driving environment (e.g. day-to-night shifts, weather shifts) that are most common in real-world driving scenarios. 
Specifically, we apply augmentations to the source domain using pre-trained style transfer\cite{jiang2020tsit} to generate styled domains for each variation. 
We define these augmented data as \textit{Weather-Augmented Data (WAD)} and through this dataset, we acquire domain-specific knowledge in advance. 
Note that this process is not conducted every time during the warm-up process, but only set once when setting the source domain.
More details are in the supplemental. 

\textbf{Domain Discriminator.}     
As we encounter unlabeled, domain-agnostic images in the CTTA situation, we need to define their pseudo-domain label to process their knowledge input-dependently. 
Therefore, we adopted a lightweight Domain Discriminator (DD) to aid the adaptive domain-wise process at CTTA. 
When we train DD, it receives the multi-domain images as input and predicts the pseudo-domain labels.
Note that this part rapidly operates like \textit{an auxiliary head} and does not affect the main forward process.
After finishing the slight training at warm-up, we \textit{freeze} it at the test-time adaptation process and utilize its inference results per each continuous image. 
% To guarantee the domain-wise process, we use a lightweight domain discriminator to classify the relevant domain knowledge (i.e., routers). 

\textbf{Multi-Domain Warm-up.}
Building upon the above process, we go through a slight warm-up process as done in previous works~\cite{ecotta, eata, lim2023ttn, choi2022improving, liu2021ttt++, adachi2022covariance, krause2010discriminative, jung2023cafa} before deploying CTTA.
Although some studies~\cite{cotta} argue that this process should be restricted due to privacy concerns and legal constructs, we believe that this is less of a problem for autonomous driving scenarios in which we have access to abundant public dashcam videos. 
Furthermore, current CTTA frameworks use a frozen backbone pre-trained from the clean dataset, such as ~\cite{cityscapes}, where the data only contains biased domains like sunny weather or German cities. 
To deal with these biases and initialize our sub-modules, we adopt a simple warm-up with the augmented pre-built dataset. 
During the warm-up, we only activate Domain Discriminator and each MoDLoRA layer which we describe next.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Input-dependent Online Blending of Experts}     

\textbf{Mixture of Domain Low-Rank Adapters.}
To address the aforementioned challenges for the efficient CTTA, we propose a Mixture-of-Domain Low-Rank Adapter (MoDLoRA) that constructs experts as domain adapters motivated by a Mixture-of-Experts (MoE) structure.
Our MoDLoRA layer consists of a set of $N$ lightweight low-rank adapter (i.e., experts), $A_1$, $A_2$, ..., $A_N$, each consisting of two feed-forward networks and an activation function, $\bm{W}^{down}$,$\bm{W}^{up}$, and $\sigma(\cdot)$, respectively. 
If the adapter is activated, it maps the input $\bm{x}$ into the low dimensional space by projection operation with $\bm{W}^{down}$. And, after regularizing the features with a non-linear activation function $\sigma$, it recovers the features to the original dimension using $\bm{W}^{up}$:

% \begin{equation}
% \bm{x}\leftarrow \bm{x}+\sigma(\bm{x}\bm{W}^{down})\bm{W}^{up}.
% \end{equation}

However, updating all adapters during CTTA is computationally inefficient and does not fully leverage the benefits of a modularized structure in addressing challenges of \textit{subordinate adaptation} and \textit{domain forgetting}. 
As shown in \Cref{fig:moda}, here, we introduce \textit{$D$ independent domain-wise router} $G_1$, $G_2$..$G_D$ to loosely cluster adapters of the model with similar domain knowledge by selecting $K$ adapter per layer. 
Each router $G_d$ is parameterized by $\bm{W}_g^d$ and $\bm{W}_{noise}^d$. 
These trainable clustering functions allow the model to activate their own set of adapters, which are specialized to specific domain knowledge. 
We note that this is crucial since a single router-based router with the same selection policy do not estimate the group adapters over multiple layers for relevant domains, resulting in less interpretable and degenerated performance.


% Through the  objective of Sparse-MoE is to maintain FLOPs by conditionally activating them according to the routing network $G(x)$. and 
% The output of the MoE layer $h(x)$ is the weighted sum of $N$ outputs from each expert $E_i$, where weights are determined by the output of routing network $G^i(x)$ which is $\sum_{i=1}^N G^i(x) = 1$.

Based on the $G_d$, we selectively update the activated adapters associated with a specific domain representation, preventing the unintended shifts of irrelevant domain knowledge during new domain adaptation. Also, our multi-router-based design is able to accelerate adaptation to the current domain, avoiding interference from knowledge transfer of unrelated domain features. 
Given the input $\bm{x}$, our proposed MoDLoRA adapter obtains the domain-adaptive features as follows:

% \begin{align}
% \small 
% \begin{split}
% P^i(\bm{x})=\text{Softmax}\left(\bm{x}\bm{W}^i_g+N\left(0,1\right)\cdot\text{\text{Softplus}}\left(\bm{x}\bm{W}^i_{noise}\right)\right) 
% \end{split}
% \end{align}

% \begin{equation}
% G_d(\bm{x})=\text{TopK}\left(\left\{P^1(\bm{x}), P^2(\bm{x}), ..., P^D(\bm{x})\right\}\right)
% \end{equation}

% \begin{align}
% \small 
% \begin{split}
% % P^i(\bm{x})=\bm{x}\bm{W}^i_g+N\left(0,1\right)\cdot\text{\text{Softplus}}\left(\bm{x}\bm{W}^i_{noise}\right) 
% \end{split}
% \end{align}

\begin{equation}
P_d(\bm{x})=\bm{x}\bm{W}^d_g+N\left(0,1\right)\cdot\text{\text{Softplus}}\left(\bm{x}\bm{W}^d_{noise}\right) 
\end{equation}

\begin{equation}
% G_d(\bm{x})=\text{Softmax}\left(\text{TopK}\left(\left\{P^1(\bm{x}), P^2(\bm{x}), ..., P^N(\bm{x})\right\}\right)\right)
G_d(\bm{x})=\text{Softmax}\left(TopK\left( P_d(\bm{x}) \right) \right) 
\end{equation}

\begin{equation}
h_d(\bm{x})=\sum_{i=1}^NG_d^i(\bm{x})\cdot\sigma(\bm{x}\bm{W}_i^{down})\bm{W}_i^{up}   
\end{equation}

We inject MoDLoRA layers at the top of each block of the pre-trained ViT backbone like plug-in-play modules. 
Given a specific domain $d$'s input representation $\bm{x}$, MoDLoRA layer conducts the following transformations:

\begin{equation}
\bm{x} \leftarrow \bm{x} + h_d(\bm{x}).
\end{equation}


% \begin{figure}[t]
%     \centering
%     {\includegraphics[width=1.0\linewidth]{./fig_v2/concept_fig.pdf}}
%     \caption{\textbf{Overall framework.} We illustrated our overall domain-adaptive framework, including input-dependent domain estimation with Domain Discriminator (DD).}
%     \label{fig:overall}
%     \vspace{-0.3cm}
% \end{figure}

% As shown in Fig~\ref{fig:moda}, 
\begin{figure}[t]
    \centering
    {\includegraphics[width=1.0\linewidth]{./fig_v2/moda_layer_v2.pdf}}
    \caption{\textbf{Details of Mixture-of-Domain Low-Rank Adapters (MoDLoRA).} Our MoDLoRA consists of domain-specific routers and low-rank adapters. $G_D$ router selects the $topK$ probable adapters and sparsely activates domain knowledge. Also, $P(A,D)$ is obtained and utilized to aggregate the mutual information between adapters and domains.}
    \label{fig:moda}
    \vspace{-0.3cm}
\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Sparsified Knowledge transfer with Adaptive Domain Experts} 
\textbf{Maximizing Mutual Loss.}
Our goal is to facilitate domain-wise knowledge through the cooperation and specialization of multiple adapters. %ensuring domain dependency. 
Inspired by ~\cite{modsquad}, we propose a domain-wise mutual loss to enhance the mutual interaction between each domain adapter. 
Since we interpret $G_d^i(\bm{x})$ as an assignment weight with specific domain $D_d$ from the $i$-th adapter $A_i$, we obtain $P(A_i|D_d)$ from all of the adapters and domains in each MoDLoRA layer. 
This conditional probability refers to the frequency with which $A_i$ is assigned to each domain $D_d$. 
% This refers to the conditional probability that a specific domain $d$ input instance is assigned to a specific $m$th adapter. 
For the entire domain and $N$ adapters, we collect $P(A_i|D_d)$ and also calculate $P(A_i, D_d)$ using the definition of conditional probability. 
\begin{equation}
P(A_i, D_d) = P(A_i|D_d) \cdot P(D_d)
\end{equation}
where $P(D_d)$ denotes the frequency of encountering the domain $D_d$. Since it is hard to define $P(D_d)$ in a real-world scenario, we assume a uniform distribution over $P(D_d)$. 
We then define the mutual information between the domain and adapter as negative entropy of $P(A_i, D_d)$ and maximize $\Theta(D;A)$ to ensure strong dependency across them.

\begin{equation}
\Theta(D;A)=\sum_i^N\sum_d^DP(A_i, D_d)\cdot logP(A_i, D_d)
\end{equation}


Therefore, the total loss we use in the warm-up process is formulated below. Except for original cross-entropy loss $L_{seg}$ for segmentation, we include an additional cross-entropy loss $L{d}$ for domain discriminator, and mutual loss $\Theta(D;A)$: 

\begin{equation}
L_{warm} = L_{seg} + \lambda_dL_{d} - \lambda_m\Theta(D;A)
\end{equation}

{where $\lambda_d$, $\lambda_m$ denotes the balance term for each loss.
% loss weights, and we set them as 1.0, 0.1, 0.0005 respectively. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Entropy Minimization with MoDLoRA}    % tentative 
% \daeun{considering order..}
Most of the preliminary work~\cite{tent, ecotta, eata} operates as a self-training manager, and adaptation is performed using entropy minimization.
Following these works, we also utilize the entropy minimization using $H(\hat{y_t}) = -\sum_{c}^{}p(\hat{y_t})logp(\hat{y_t})$. As a way to prevent forgetting and error accumulation more stably, we proceed with the stochastic restoration~\cite{cotta} and filtering based on the confidence of the pseudo labels.
Therefore, the entropy-based CTTA loss is obtained as follows:

\begin{equation}
L_{tta}=\mathds{1}_{\{{H(\hat{y_t})<\kappa}\} \cap \{\hat{y}_t-\hat{y}_0>0\}} \cdot H(\hat{y_t}),
\end{equation}
where $\hat{y_t}$ is the output prediction in the current adaptation stage $t$, $\hat{y_0}$ is the output prediction from the source model, $\kappa$ is the pre-defined entropy threshold, and $\mathds{1}\{\cdot\}$ denotes an indicator function.

==> table/ablation.tex <==
% \begin{table}[h]
% \centering
% \renewcommand{\arraystretch}{1.2}
% \setlength{\tabcolsep}{.3em}
% \caption{\textbf{Ablation study for each model part.} \daeun{It will be modified soon}}
% \label{tab:ablation}
%     {\footnotesize
%     \begin{tabular}{l|llll|c}
%     \hline & \multicolumn{1}{c}{DD} & \multicolumn{1}{c}{MoDA_{random}} & \multicolumn{1}{c}{MoDA_{topk}} & \multicolumn{1}{c|}{Mutual} & Total Mean \\ \hline
%     $E_1$ &  &  &  &  & 51.14 \\
%     $E_2$ & \ding{52} &  &  &  & 51.18 \\
%     $E_3$ &  & \ding{52} &  &  & 53.48 \\
%     $E_4$ & \ding{52} & \ding{52} &  &  & 53.53 \\
%     $E_5$ & \ding{52} &  & \ding{52} &  & 53.87 \\ 
%     \rowcolor[HTML]{EFEFEF}
%     $E_6$ & \ding{52} &  & \ding{52} & \ding{52} & \textbf{54.27} \\ \hline
%     \end{tabular}}
% \end{table}


%%% Ver.2 
% \begin{table}[h]
% \centering
% \renewcommand{\arraystretch}{1.2}
% \setlength{\tabcolsep}{.5em}
% \caption{\textbf{Ablation study for each model part.} \daeun{bottom_k is adding}}
% \resizebox{\columnwidth}{!}{%
% {\footnotesize
% \begin{tabular}{c|cccc|c}
% \hline
%  & DD & MoDA_{top_k} & MoDA_{bottom_k} & Mutual loss & Avg \\ \hline
% E_1 &  &  &  &  & 51.14 \\
% E_2 & \ding{52} &  &  &  & 51.18 \\
% E_3 & \ding{52} & \ding{52} &  &  & 53.87 \\
% E_4 & \ding{52} & \ding{52} &  & \ding{52} & \textbf{54.27} \\
% E_5 & \ding{52} &  & \ding{52} &  &  \\ \hline
% \end{tabular}%
% }
% \label{ref:ablation}
% \end{table}

%%%%%%%%%%%%%%%%%%%%%% subfigure %%%%%%%%%%%%%%%%%%%%%% -> 양 옆에 가로로 배치하고 싶은데 잘 안되네요 ..
% \begin{figure}[h]
% \centering

% % figure 
%   \begin{subfigure}[]{0.33\textwidth}
%   \centering
%   \caption{\textbf{Ablation of the number of experts and k values.} }
%   \includegraphics[width=.9\columnwidth]{./fig/k_effect.eps}
%   \label{fig:k_effect}
%   \end{subfigure}

% % table 
% \begin{subtable}[]{0.33\textwidth}
%     \centering
%     \caption{\textbf{Ablation study for each model part.} \daeun{bottom-k is adding}}
%     \renewcommand{\arraystretch}{1.2}
%     \setlength{\tabcolsep}{.5em}
%     \resizebox{\columnwidth}{!}{%
%     {\footnotesize
%     \begin{tabular}{c|cccc|c}
%     \hline
%      & DD & MoDA_{top_k} & MoDA_{bottom_k} & Mutual loss & Avg \\ \hline
%     E_1 &  &  &  &  & 51.14 \\
%     E_2 & \ding{52} &  &  &  & 51.18 \\
%     E_3 & \ding{52} & \ding{52} &  &  & 53.87 \\
%     E_4 & \ding{52} & \ding{52} &  & \ding{52} & \textbf{54.27} \\
%     E_5 & \ding{52} &  & \ding{52} &  &  \\ \hline
%     \end{tabular}%
%     }}
%     \label{ref:ablation}
% \end{subtable}
% \label{fig:ablation}
% \end{figure}




==> table/hidden_dim.tex <==
\begin{table}[t]
\centering
% \vspace{2mm}
\renewcommand{\arraystretch}{1.7}
\caption{\textbf{Ablation study of different hidden dimensions of adapters.} We conducted an ablation study on the number of experts\&k and the hidden dimension of each adapter in BECoTTA for scenario (ii). Note that BECoTTA can have flexible parameters depending on the architecture configuration. \daeun{will be modified}}
% \resizebox{\columnwidth}{!}{%
\begin{tabular}{c|cc|ccccc|c}
\hline  
\textbf{Parameters} & \multicolumn{1}{c|}{\textbf{Experts}} & \textbf{Hidden dim} & B-Clear & A-Fog & A-Night & A-Snow & B-Over & Avg \\ \hline \hline
\textbf{378,144} & \multicolumn{1}{c|}{Exp6, K3} & [0,0,0,16] & 44.31 & 69.15 & 40.10 & 57.52 & 49.64 & 52.14 \\
\textbf{779,916 }& \multicolumn{1}{c|}{Exp6, K3} & [2,4,10,16] & \textbf{45.45} & \textbf{70.77} & \textbf{42.62} & \textbf{59.66} & \textbf{50.76 }& \textbf{53.85} \\ \hline
\rowcolor[HTML]{EFEFEF} 
3,469,312 & \multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{EcoTTA}~\cite{ecotta}} & 44.64 & 70.21 & 41.68 & 58.02 & 49.94 & 52.90 \\ \hline
\textbf{9,109,056 }& \multicolumn{1}{c|}{Exp6, K3} & [32,64,160,256] & 45.45 & 70.61 & 44.32 & 59.40 & 50.61 & 54.08 \\
\textbf{15,181,760} & \multicolumn{1}{c|}{Exp10, K4} & [32,64,160,256] & 46.17 & \textbf{71.30} & 43.47 & 60.63 & 51.18 & 54.55 \\ \hline
\rowcolor[HTML]{EFEFEF} 
477,805,276 & \multicolumn{2}{c|}{\cellcolor[HTML]{EFEFEF}\textbf{CoTTA w/ full update}~\cite{cotta}} & \textbf{46.42} & 70.64 & \textbf{45.70} & \textbf{61.20} & \textbf{51.32} & \textbf{55.06 }\\ \hline
\end{tabular}%
% }
\label{ref:hidden_dim}
\vspace{-3mm}
\end{table}



==> table/ten_table_v1.tex <==
\begin{table*}[t]
\centering
\caption{\textbf{Quantitative results of \textit{CDS-Hard (imbalanced weather \& area shifts)}} We devised a novel scenario encompassing imbalanced weather and area shifts. We presented performance results for both \textit{without WAD} and \textit{with WAD} across the overall baselines. Given that our BECoTTA can take on different versions based on the number of experts and hidden dimensions, we reported both $M$ and $L$ versions, corresponding to variations in the number of parameters.}

\setlength{\tabcolsep}{.2em}
\resizebox{\linewidth}{!}{%

{\tiny
\begin{tabular}{lcc|cccccc|cccccc}
% \toprule
\multicolumn{3}{c|}{\textbf{Round}} & \multicolumn{6}{c|}{\textbf{1}} & \multicolumn{6}{c}{\textbf{4}} \\ \hline
\multicolumn{1}{c|}{Method} & \textbf{Parameters} & \textbf{Memory(MB)} & B-Clear & A-Fog & A-Night & A-Snow & \multicolumn{1}{c|}{B-Overcast} & Mean & B-Clear & A-Fog & A-Night & A-Snow & \multicolumn{1}{c|}{B-Overcast} & Mean \\ \hline

\multicolumn{1}{l|}{Source only} & - &  105.76  & 41.0 & 64.4 & 33.4 & 54.3 & \multicolumn{1}{c|}{46.3} & 47.9 
& 41.0  & 64.4  & 33.4  & 54.3 
& \multicolumn{1}{c|}{46.3} & 47.9  \\ 
\multicolumn{1}{l|}{~~~~~~~~~~+ \textit{WAD}} & - & 105.76 & 43.6 & 68.7 & 44.5 & 59.0 & \multicolumn{1}{c|}{48.7} & 52.9 & 
 43.6 & 68.7  & 44.5  & 59.0  & \multicolumn{1}{c|}{48.7} &  52.9 \\ \hline 

\multicolumn{1}{l|}{CoTTA~\cite{cotta}} & \textit{54,727,372} & 533.81 & 43.3 & 67.3 & 34.8 & 56.9 & \multicolumn{1}{c|}{48.8} & 50.2 & 
 43.3 & 67.3  & 34.8 & 56.9  & \multicolumn{1}{c|}{48.8} &   50.2 \\
\multicolumn{1}{l|}{~~~~~~~~~~+ \textit{WAD}} & \textit{54,727,372} & 533.81 & 46.4 & 70.6 & 45.7 & 61.2 & \multicolumn{1}{c|}{51.3} & 55.0 & 
46.1  & 70.5  &  45.6 &  61.1 & \multicolumn{1}{c|}{51.2} &  54.9 \\ \hline 

\multicolumn{1}{l|}{TENT~\cite{tent}} & \textit{27,520} & 105.88 & 41.1 & 64.9 & 33.2 & 54.3 & \multicolumn{1}{c|}{46.3} & 47.9 & 
38.6 & 62.0 &28.3& 49.1& \multicolumn{1}{c|}{41.6} &  43.9 \\
  % &  &   &   & \multicolumn{1}{c|}{ } &     \\
\multicolumn{1}{l|}{~~~~~~~~~~+ \textit{WAD}} & \textit{27,520} & 105.88 & 43.7 & 68.5 & 44.6 & 59.0 & \multicolumn{1}{c|}{48.3} & 52.8 & 
 41.4 & 64.6  &  40.7 & 53.5  & \multicolumn{1}{c|}{44.8} &  49.0  \\ \hline 
    
\multicolumn{1}{l|}{SAR~\cite{sar}} & \textit{27,520} & 105.88 & 41.0 & 64.5 & 33.4 & 54.5 & \multicolumn{1}{c|}{46.6} & 48.0 
& 41.4 & 64.8 & 33.1 & 54.8 & \multicolumn{1}{c|}{46.9} &  48.2 \\
\multicolumn{1}{l|}{~~~~~~~~~~+ \textit{WAD}} & \textit{27,520} & 105.88 & 43.6 & 68.6 & 44.5 & 59.1 & \multicolumn{1}{c|}{48.7} & 52.9 & 
43.7 & 68.3 & 44.0 & 59.0 & \multicolumn{1}{c|}{48.7} & 52.7  \\ \hline
    
\multicolumn{1}{l|}{EcoTTA~\cite{ecotta}} & \textit{3,469,312} & 251.21 & 44.1 & 69.6 & 35.3 & 58.2 & \multicolumn{1}{c|}{49.6} & 51.3 
& 44.0 &69.2 & 34.7& 57.9 & \multicolumn{1}{c|}{49.1} &  50.9\\ 

\multicolumn{1}{l|}{~~~~~~~~~~+ \textit{WAD}} & \textit{3,469,312} & 251.21 & 44.6 & 70.2 & 41.6 & 58.0 & \multicolumn{1}{c|}{49.9} & 52.9 
& 43.7 & 69.1 & 36.4 & 56.8 &\multicolumn{1}{c|}{48.3} & 50.8  \\ \hline

\multicolumn{1}{l|}{\cellcolor{gg}Ours-M} & 
\cellcolor{gg}\textit{630,156} & 
\cellcolor{gg}\textbf{231.36} & 
\cellcolor{gg}43.8 &
\cellcolor{gg}68.8 &
\cellcolor{gg}34.9 &
\cellcolor{gg}57.9 &
\multicolumn{1}{c|}{\cellcolor{gg}49.2} & 
\cellcolor{gg}50.9 & 
\cellcolor{gg}43.7 & 
\cellcolor{gg}68.9 & 
\cellcolor{gg}34.8 & 
\cellcolor{gg}57.9 & 
\multicolumn{1}{c|}{\cellcolor{gg}49.3} &
\cellcolor{gg} 50.9 \\

\multicolumn{1}{l|}{\cellcolor{gg}~~~~~~~~~~+ \textit{WAD}} &
\cellcolor{gg}\textit{779,916} & 
\cellcolor{gg}\textbf{234.02} & 
\cellcolor{gg}45.6 & 
\cellcolor{gg}70.8 & 
\cellcolor{gg}42.6 & 
\cellcolor{gg}59.7 & 
\multicolumn{1}{c|}{\cellcolor{gg}50.8} & 
\cellcolor{gg}53.9 & 
\cellcolor{gg}45.6 & 
\cellcolor{gg}70.8 & 
\cellcolor{gg}42.6 & 
\cellcolor{gg}59.5 & 
\multicolumn{1}{c|}{\cellcolor{gg}50.8} & 
\cellcolor{gg} 53.8\\ \hline 

% \multicolumn{1}{l|}{\cellcolor{ggg} Ours-L} &
% \cellcolor{ggg} \textit{1,208,448} &
% \cellcolor{ggg} 336.68 & 
% \cellcolor{ggg} \textbf{44.1} &
% \cellcolor{ggg} 68.8 &
% \cellcolor{ggg} \textbf{35.3} &
% \cellcolor{ggg} \textbf{58.3} &
% \multicolumn{1}{c|}{\cellcolor{ggg}49.4} &
% \cellcolor{ggg} 51.2 & 
% \cellcolor{ggg} 44.0 &
% \cellcolor{ggg} 68.7 &
% \cellcolor{ggg} 35.3 &
% \cellcolor{ggg} 58.4 &
% \multicolumn{1}{c|}{\cellcolor{ggg}49.4} &
% \cellcolor{ggg} 51.1 \\

% \multicolumn{1}{l|}{\cellcolor{ggg}~~~~~~~~~~+ \textit{WAD}} &
% \cellcolor{ggg} \textit{1,518,176} &
% \cellcolor{ggg} 342.77 & 
% \cellcolor{ggg} \textbf{46.2} &
% \cellcolor{ggg} \textbf{71.3} &
% \cellcolor{ggg} \textbf{43.5} &
% \cellcolor{ggg} \textbf{60.6} &
% \multicolumn{1}{c|}{\cellcolor{ggg}\textbf{51.2}} &
% \cellcolor{ggg} \textbf{54.6} &
% \cellcolor{ggg} \textbf{46.2} &
% \cellcolor{ggg} \textbf{71.3} &
% \cellcolor{ggg} \textbf{43.6} &
% \cellcolor{ggg} \textbf{60.7} &
% \multicolumn{1}{c|}{\cellcolor{ggg}\textbf{50.9}} &
% \cellcolor{ggg} \textbf{54.5}  \\ \hline
% \bottomrule
\end{tabular}%
}
}

\vspace{.5cm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\resizebox{\linewidth}{!}{%
{\tiny
\begin{tabular}{lcc|cccccc|cccccc}
% \toprule
\multicolumn{3}{c|}{\textbf{Round}} & \multicolumn{6}{c|}{\textbf{7}} & \multicolumn{6}{c}{\textbf{10}} \\ \hline
\multicolumn{1}{c|}{Method} & \textbf{Parameters} & \textbf{Memory(MB)} & B-Clear & A-Fog & A-Night & A-Snow & \multicolumn{1}{c|}{B-Overcast} & Mean & B-Clear & A-Fog & A-Night & A-Snow & \multicolumn{1}{c|}{B-Overcast} & Mean \\ \hline

\multicolumn{1}{l|}{Source only} & - &  105.76 
& 41.0 & 64.4 & 33.4 & 54.3 & \multicolumn{1}{c|}{46.3} & 47.9 
& 41.0 & 64.4 & 33.4 & 54.3 & \multicolumn{1}{c|}{46.3} & 47.9  \\ 

\multicolumn{1}{l|}{~~~~~~~~~~+ \textit{WAD}} & - & 105.76 
& 43.6 & 68.7 & 44.5 & 59.0 & \multicolumn{1}{c|}{48.7} &  52.9 & 43.6 & 68.7 & 44.5 & 59.0 & \multicolumn{1}{c|}{48.7} & 52.9 \\ \hline 

\multicolumn{1}{l|}{CoTTA~\cite{cotta}} & \textit{54,727,372} & 533.81 
& 43.3 & 67.3 & 34.8 & 56.9 & \multicolumn{1}{c|}{48.8} & 50.2 & 43.3 & 67.3 & 34.8 & 56.9 & \multicolumn{1}{c|}{48.8} & 50.2  \\

\multicolumn{1}{l|}{~~~~~~~~~~+ \textit{WAD}} & \textit{54,727,372} & 533.81 & 
46.1 & 70.5 & 45.6 & 61.1 & \multicolumn{1}{c|}{51.2} & 54.9 
& 46.1 & 70.5 & 45.6 & 61.1 & \multicolumn{1}{c|}{51.2} & 54.9 \\ \hline 

\multicolumn{1}{l|}{TENT~\cite{tent}} & \textit{27,520} & 105.88 
&34.4 & 56.4 & 23.5 & 42.2 & \multicolumn{1}{c|}{36.7} &  38.6
% &&&&& \multicolumn{1}{c|}{} &  
& 30.9 & 51.5 & 20.4 & 37.0 & \multicolumn{1}{c|}{33.0} & 34.6   \\
\multicolumn{1}{l|}{~~~~~~~~~~+ \textit{WAD}} & \textit{27,520} & 105.88 
& 38.3 & 60.9 & 36.6 & 48.3 & \multicolumn{1}{c|}{41.3} & 45.0
& 35.8 & 57.6 & 33.6 & 44.3 & \multicolumn{1}{c|}{38.8} & 42.0  \\ \hline 
    
\multicolumn{1}{l|}{SAR~\cite{sar}} & \textit{27,520} & 105.88 
& 41.4 & 64.7 & 32.4 & 54.6 & \multicolumn{1}{c|}{46.8} & 47.9 & 
41.3 & 64.3 & 31.6 & 54.2 & \multicolumn{1}{c|}{46.6} & 47.6  \\
\multicolumn{1}{l|}{~~~~~~~~~~+ \textit{WAD}} & \textit{27,520} & 105.88 
& 43.6 & 67.9 & 43.1 & 58.6 & \multicolumn{1}{c|}{48.5} & 52.3 
& 43.4 & 67.4 & 42.2 & 58.1 & \multicolumn{1}{c|}{47.6} & 51.9  \\ \hline
    
\multicolumn{1}{l|}{EcoTTA~\cite{ecotta}} & \textit{3,469,312} & 251.21  
& 43.2 & 67.9 & 33.4 & 56.8 & \multicolumn{1}{c|}{47.9} & 49.8 
& 41.9 & 66.1 & 31.5 & 55.3 & \multicolumn{1}{c|}{46.2} & 48.2  \\ 

\multicolumn{1}{l|}{~~~~~~~~~~+ \textit{WAD}} & \textit{3,469,312} & 251.21 
& 42.3 & 67.3 & 32.1& 55.8 & \multicolumn{1}{c|}{46.7} & 48.8 &
41.1 & 65.6 & 27.0 & 53.2 & \multicolumn{1}{c|}{45.3} & 46.4  \\ \hline

\multicolumn{1}{l|}{\cellcolor{gg}Ours-M} & 
\cellcolor{gg}\textit{630,156} & 
\cellcolor{gg}\textbf{231.36} & 
\cellcolor{gg} 43.7&
\cellcolor{gg}68.8 &
\cellcolor{gg} 34.8&
\cellcolor{gg} 57.9&
\multicolumn{1}{c|}{\cellcolor{gg}49.1} & 
\cellcolor{gg} 50.8 & 
\cellcolor{gg}43.7 & 
\cellcolor{gg}68.8 & 
\cellcolor{gg}34.5 & 
\cellcolor{gg}57.9 & 
\multicolumn{1}{c|}{\cellcolor{gg}49.2} &
% \cellcolor{gg}50.9 &
\cellcolor{gg}50.9 \\

\multicolumn{1}{l|}{\cellcolor{gg}~~~~~~~~~~+ \textit{WAD}} &
\cellcolor{gg}\textit{779,916} & 
\cellcolor{gg}\textbf{234.02} & 
\cellcolor{gg} 45.6 & 
\cellcolor{gg} 70.6& 
\cellcolor{gg} 42.6& 
\cellcolor{gg} 59.6& 
\multicolumn{1}{c|}{\cellcolor{gg}50.8} & 
\cellcolor{gg} 53.8& 
\cellcolor{gg}45.6 & 
\cellcolor{gg}70.7 & 
\cellcolor{gg}42.5 & 
\cellcolor{gg}59.5 & 
\multicolumn{1}{c|}{\cellcolor{gg}50.8} & 
% \cellcolor{gg}53.9 & 
\cellcolor{gg}53.9 \\ \hline 

% \multicolumn{1}{l|}{\cellcolor{ggg} Ours-L} &
% \cellcolor{ggg} \textit{1,208,448} &
% \cellcolor{ggg} 336.68 & 
% \cellcolor{ggg} 44.1 &
% \cellcolor{ggg} 68.8 &
% \cellcolor{ggg} 35.2 &
% \cellcolor{ggg} 58.3 &
% \multicolumn{1}{c|}{\cellcolor{ggg}49.3} &
% \cellcolor{ggg} 51.1 & 
% \cellcolor{ggg} \textbf{44.1} &
% \cellcolor{ggg} \textbf{68.8} &
% \cellcolor{ggg} \textbf{35.3} &
% \cellcolor{ggg} \textbf{58.4} &
% \multicolumn{1}{c|}{\cellcolor{ggg}\textbf{49.3}} &
% \cellcolor{ggg} \textbf{51.2} \\

% \multicolumn{1}{l|}{\cellcolor{ggg}~~~~~~~~~~+ \textit{WAD}} &
% \cellcolor{ggg} \textit{1,518,176} &
% \cellcolor{ggg} 342.77 & 
% \cellcolor{ggg} \textbf{46.3} &
% \cellcolor{ggg} \textbf{71.2} &
% \cellcolor{ggg} \textbf{43.5} &
% \cellcolor{ggg} \textbf{60.7} &
% \multicolumn{1}{c|}{\cellcolor{ggg}\textbf{50.7}} &
% \cellcolor{ggg} \textbf{54.4} &
% \cellcolor{ggg} \textbf{46.3} &
% \cellcolor{ggg} \textbf{71.5} &
% \cellcolor{ggg} \textbf{43.6} &
% \cellcolor{ggg} \textbf{60.7} &
% \multicolumn{1}{c|}{\cellcolor{ggg}\textbf{51.1}} &
% \cellcolor{ggg} \textbf{54.6}  \\
% \bottomrule 
\hline
\end{tabular}%
}
}

\label{table:more_2}
\end{table*}


% \clearpage
% \bibliography{main}

% {
%     \small
%     \bibliographystyle{ieeenat_fullname}
%     \bibliography{main}
% }


% \end{document}




==> table/wo_ours_backup.tex <==
\begin{table*}[h]
\centering
\renewcommand{\arraystretch}{1.25}
\caption{\textbf{Results on \textit{CDS-Hard (imbalanced weather \& area shifts)}.} We devise a novel scenario encompassing imbalanced weather and area shifts. We present performance results for both \textit{w/o WAD} and \textit{w/ WAD} across the overall baselines. We report $S$, $M$, and $L$ versions for our BECoTTA based on the number of parameters. }
\vspace{-0.05in}
\setlength{\tabcolsep}{.2em}
\resizebox{\linewidth}{!}{%
\begin{tabular}{clcc|cccccc|cccccc|c}
\toprule
\multicolumn{4}{c|}{Round} & \multicolumn{6}{c|}{\textbf{1}} & \multicolumn{6}{c|}{\textbf{10}} & \multirow{2}{*}{$\Delta$} \\ \cline{1-16}

\multicolumn{1}{c|}{Init} & \multicolumn{1}{c|}{Method} & Parameters & Init update & B-Clear & A-Fog & A-Night & A-Snow & \multicolumn{1}{c|}{B-Overcast} & Mean & \multicolumn{1}{l}{B-clear} & \multicolumn{1}{l}{A-Fog} & \multicolumn{1}{l}{A-Night} & \multicolumn{1}{l}{A-Snow} & \multicolumn{1}{l|}{B-Overcast} & \multicolumn{1}{c|}{Mean} &  \\ \hline \hline

\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{Source only} & - & - &41.0 & 64.4 & 33.4 & 54.3 & \multicolumn{1}{c|}{46.3} & 47.9 & 41.0 & 64.4 & 33.4 & 54.3 & \multicolumn{1}{c|}{46.3} & 47.9 & +0.0 \\ 

\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{CoTTA~\cite{cotta}} & \textbf{54.72M} & - & 43.3 & 67.3 & 34.8 & 56.9 & \multicolumn{1}{c|}{48.8} & 50.2 & 43.3 & 67.3 & 34.8 & 56.9 & \multicolumn{1}{c|}{48.8} & 50.2 & +0.0 \\

\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{TENT~\cite{tent}} & 0.02M & - & 41.1 & 64.9 & 33.2 & 54.3 & \multicolumn{1}{c|}{46.3} & 47.9 & 30.9 & 51.5 & 20.4 & 37.0 & \multicolumn{1}{c|}{33.0} & 34.6 & \textcolor{red}{-13.3} \\
    
\multicolumn{1}{l|}{\textit{w/o WAD}} & \multicolumn{1}{l|}{SAR~\cite{sar}} & 0.02M &  - & 41.0 & 64.5 & 33.4 & 54.5 & \multicolumn{1}{c|}{46.6} & 48.0 & 41.3 & 64.3 & 31.6 & 54.2 & \multicolumn{1}{c|}{46.6} & 47.6 & \textcolor{red}{-0.4} \\
    
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{EcoTTA~\cite{ecotta}} & 3.46M & \textit{\textcolor{darkcerulean}{MetaNet}} & 44.1 & 69.6 & 35.3 & 58.2 & \multicolumn{1}{c|}{49.6} & 51.3 & 41.9 & 66.1 & 31.5 & 55.3 & \multicolumn{1}{c|}{46.2} & 48.2 & \textcolor{red}{-3.1} \\ 

\multicolumn{1}{l|}{}& \multicolumn{1}{l|}{\cellcolor{g}BECoTTA (Ours)-S} &
\cellcolor{g}0.09M & 
\cellcolor{g}\textit{\textcolor{darkcerulean}{MoDE}} & 
\cellcolor{g}42.9 &
\cellcolor{g}68.5 &
\cellcolor{g}35.0 &
\cellcolor{g}57.2 &
\multicolumn{1}{c|}{\cellcolor{g}47.8} &
\cellcolor{g}50.5 &
\cellcolor{g}43.0 &
\cellcolor{g}69.5 &
\cellcolor{g}35.1 &
\cellcolor{g}57.3 &
\multicolumn{1}{c|}{\cellcolor{g}48.8} &
\cellcolor{g}50.7 &
\cellcolor{g}+0.1 \\

\multicolumn{1}{l|}{}& \multicolumn{1}{l|}{\cellcolor{gg}BECoTTA (Ours)-M} & 
\cellcolor{gg}0.63M &
\cellcolor{gg}\textit{\textcolor{darkcerulean}{MoDE}} & 
\cellcolor{gg}43.8 &
\cellcolor{gg}68.8 &
\cellcolor{gg}34.9 &
\cellcolor{gg}57.9 &
\multicolumn{1}{c|}{\cellcolor{gg}49.2} & 
\cellcolor{gg}50.9 & 
\cellcolor{gg}43.7 & 
\cellcolor{gg}68.8 & 
\cellcolor{gg}34.5 & 
\cellcolor{gg}57.9 & 
\multicolumn{1}{c|}{\cellcolor{gg}49.2} &
\cellcolor{gg}50.9 &
\cellcolor{gg}+0.0 \\

\multicolumn{1}{l|}{}& \multicolumn{1}{l|}{\cellcolor{ggg}BECoTTA (Ours)-L} &
\cellcolor{ggg}3.16M &
\cellcolor{ggg}\textit{\textcolor{darkcerulean}{MoDE}} & 
\cellcolor{ggg}43.9 &
\cellcolor{ggg}69.1 &
\cellcolor{ggg}35.0 &
\cellcolor{ggg}58.3 &
\multicolumn{1}{c|}{\cellcolor{ggg}50.2} &
\cellcolor{ggg}51.3 &
\cellcolor{ggg}44.0 &
\cellcolor{ggg}69.1 &
\cellcolor{ggg}35.1 &
\cellcolor{ggg}58.3 &
\multicolumn{1}{c|}{\cellcolor{ggg}50.2} &
\cellcolor{ggg}51.3 &
\cellcolor{ggg}+0.0 \\ \hline

\multicolumn{1}{l|}{}  & \multicolumn{1}{l|}{Source only} & - & \textit{\textcolor{crimson}{Full}} & 43.6 & 68.7 & 44.5 & 59.0 & \multicolumn{1}{c|}{48.7} & 52.9 & 43.6 & 68.7 & 44.5 & 59.0 & \multicolumn{1}{c|}{48.7} & 52.9 & +0.0 \\  

\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{CoTTA~\cite{cotta}} & \textbf{54.72M} & \textit{\textcolor{crimson}{Full}} & 46.4 & 70.6 & 45.7 & 61.2 & \multicolumn{1}{c|}{51.3} & 55.0 & 46.1 & 70.5 & 45.6 & 61.1 & \multicolumn{1}{c|}{51.2} & 54.9 & \textcolor{red}{-0.1} \\ 

\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{TENT~\cite{tent}} & 0.02M & \textit{\textcolor{crimson}{Full}} & 43.7 & 68.5 & 44.6 & 59.0 & \multicolumn{1}{c|}{48.3} & 52.8 & 35.8 & 57.6 & 33.6 & 44.3 & \multicolumn{1}{c|}{38.8} & 42.0 & \textcolor{red}{-10.8} \\ 

\multicolumn{1}{l|}{\textit{w/ WAD}} & \multicolumn{1}{l|}{SAR~\cite{sar}} & 0.02M & \textit{\textcolor{crimson}{Full}} & 43.6 & 68.6 & 44.5 & 59.1 & \multicolumn{1}{c|}{48.7} & 52.9 & 43.4 & 67.4 & 42.2 & 58.1 & \multicolumn{1}{c|}{47.6} & 51.9 & \textcolor{red}{-1.0} \\ 

\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{EcoTTA~\cite{ecotta}} & 3.46M & \textit{\textcolor{darkcerulean}{MetaNet}} & 44.6 & 70.2 & 41.6 & 58.0 & \multicolumn{1}{c|}{49.9} & 52.9 & 41.1 & 65.6 & 27.0 & 53.2 & \multicolumn{1}{c|}{45.3} & 46.4 & \textcolor{red}{-6.5} \\ 

% \textcolor{blue}{\scriptsize ($-6.5\%$)}

\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\cellcolor{g}BECoTTA (Ours)-S} &
\cellcolor{g}0.12M &
\cellcolor{g}\textit{\textcolor{darkcerulean}{MoDE}} & 
\cellcolor{g}44.1 &
\cellcolor{g}69.5 &
\cellcolor{g}40.1 &
\cellcolor{g}56.8 &
\multicolumn{1}{c|}{\cellcolor{g}49.1} &
\cellcolor{g}51.9 &
\cellcolor{g}44.0 &
\cellcolor{g}69.4 &
\cellcolor{g}40.1 &
\cellcolor{g}56.9 &
\multicolumn{1}{c|}{\cellcolor{g}49.1} &
\cellcolor{g}51.9 &
\cellcolor{g}+0.0 \\ 

\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\cellcolor{gg}BECoTTA (Ours)-M } &
\cellcolor{gg}0.77M & 
\cellcolor{gg}\textit{\textcolor{darkcerulean}{MoDE}} & 
\cellcolor{gg}45.6 & 
\cellcolor{gg}70.8 & 
\cellcolor{gg}42.6 & 
\cellcolor{gg}59.6 & 
\multicolumn{1}{c|}{\cellcolor{gg}\textbf{50.8}} & 
\cellcolor{gg}53.9 & 
\cellcolor{gg}45.6 & 
\cellcolor{gg}70.7 & 
\cellcolor{gg}42.5 & 
\cellcolor{gg}59.5 & 
\multicolumn{1}{c|}{\cellcolor{gg}\textbf{50.8}} & 
\cellcolor{gg}53.9 & 
\cellcolor{gg}+0.0 \\ 

\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{\cellcolor{ggg}BECoTTA (Ours)-L } &
\cellcolor{ggg}3.32M &
\cellcolor{ggg}\textit{\textcolor{darkcerulean}{MoDE}} & 
\cellcolor{ggg}\textbf{45.7} &
\cellcolor{ggg}\textbf{71.4} &
\cellcolor{ggg}\textbf{43.7} &
\cellcolor{ggg}\textbf{59.6} &
\multicolumn{1}{c|}{\cellcolor{ggg}50.5} &
\cellcolor{ggg}\textbf{54.2} &
\cellcolor{ggg}\textbf{45.7} &
\cellcolor{ggg}\textbf{71.3} &
\cellcolor{ggg}\textbf{43.7} &
\cellcolor{ggg}\textbf{59.6} &
\multicolumn{1}{c|}{\cellcolor{ggg}50.6} &
\cellcolor{ggg}\textbf{54.2} &
\cellcolor{ggg}\textbf{+0.0}\\
\bottomrule
\end{tabular}%
}
\label{ref:main2_v2}
\vspace{-0.1in}
\end{table*}


% \textcolor{red}{\scriptsize ($\bm +0.0$)}

==> table/wo_ours_memory.tex <==
\begin{table*}[h]
\centering
\renewcommand{\arraystretch}{1.25}
\caption{\textbf{Quantitative results of \textit{CDS-(ii) imbalanced weather \& area shifts} scenario.} We devised a novel scenario encompassing imbalanced weather and area shifts. We presented performance results for both \textit{w/o WAD} and \textit{w/ WAD} across the overall baselines. Given that our BECoTTA can take on different versions based on the number of experts and hidden dimensions, we reported both $M$ and $L$ versions, corresponding to variations in the number of parameters.}

\setlength{\tabcolsep}{.2em}
\resizebox{\linewidth}{!}{%
\begin{tabular}{lccc|cccccc|cccccc|c}
\toprule
\multicolumn{4}{c|}{Round} & \multicolumn{6}{c|}{\textbf{1}} & \multicolumn{6}{c|}{\textbf{10}} & \multirow{2}{*}{Total Mean} \\ \cline{1-16}

\multicolumn{1}{c|}{Method} & Parameters & Memory & Init update & B-Clear & A-Fog & A-Night & A-Snow & \multicolumn{1}{c|}{B-Overcast} & Mean & \multicolumn{1}{l}{B-clear} & \multicolumn{1}{l}{A-Fog} & \multicolumn{1}{l}{A-Night} & \multicolumn{1}{l}{A-Snow} & \multicolumn{1}{l|}{B-Overcast} & \multicolumn{1}{l|}{Mean} &  \\ \hline \hline

\multicolumn{1}{l|}{Source only} & - & - & 105.7MB & 41.0 & 64.4 & 33.4 & 54.3 & \multicolumn{1}{c|}{46.3} & 47.9 & 41.0 & 64.4 & 33.4 & 54.3 & \multicolumn{1}{c|}{46.3} & 47.9 & 47.9 \\ 

\multicolumn{1}{l|}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~+ \textit{w/WAD}} & - & - & \textit{\textcolor{crimson}{Full}} & 43.6 & 68.7 & 44.5 & 59.0 & \multicolumn{1}{c|}{48.7} & 52.9 & 43.6 & 68.7 & 44.5 & 59.0 & \multicolumn{1}{c|}{48.7} & 52.9 & 52.9 \\ \hline 

\multicolumn{1}{l|}{CoTTA~\cite{cotta}} & \textit{\textbf{54.72M}} & \textit{\textbf{533.8MB}}& - & 43.3 & 67.3 & 34.8 & 56.9 & \multicolumn{1}{c|}{48.8} & 50.2 & 43.3 & 67.3 & 34.8 & 56.9 & \multicolumn{1}{c|}{48.8} & 50.2 & 50.3 \\
\multicolumn{1}{l|}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~+ \textit{w/WAD}} & \textit{\textbf{54.72M}} & \textit{\textbf{533.8MB}} & \textit{\textcolor{crimson}{Full}} & 46.4 & 70.6 & 45.7 & 61.2 & \multicolumn{1}{c|}{51.3} & 55.0 & 46.1 & 70.5 & 45.6 & 61.1 & \multicolumn{1}{c|}{51.2} & 54.9 & 54.9 \\ \hline 

\multicolumn{1}{l|}{TENT~\cite{tent}} & \textit{0.02M} & \textit{105.8MB} & - & 41.1 & 64.9 & 33.2 & 54.3 & \multicolumn{1}{c|}{46.3} & 47.9 & 30.9 & 51.5 & 20.4 & 37.0 & \multicolumn{1}{c|}{33.0} & 34.6 & 42.7 \\

\multicolumn{1}{l|}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~+ \textit{w/WAD}} & \textit{0.02M} & \textit{105.8MB} &  \textit{\textcolor{crimson}{Full}} & 43.7 & 68.5 & 44.6 & 59.0 & \multicolumn{1}{c|}{48.3} & 52.8 & 35.8 & 57.6 & 33.6 & 44.3 & \multicolumn{1}{c|}{38.8} & 42.0 & 48.4 \\ \hline 
    
\multicolumn{1}{l|}{SAR~\cite{sar}} & \textit{0.02M} &  \textit{105.8MB} &  - & 41.0 & 64.5 & 33.4 & 54.5 & \multicolumn{1}{c|}{46.6} & 48.0 & 41.3 & 64.3 & 31.6 & 54.2 & \multicolumn{1}{c|}{46.6} & 47.6 & 47.9 \\
\multicolumn{1}{l|}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~+ \textit{w/WAD}} & \textit{0.02M} & \textit{105.8MB} & \textit{\textcolor{crimson}{Full}} & 43.6 & 68.6 & 44.5 & 59.1 & \multicolumn{1}{c|}{48.7} & 52.9 & 43.4 & 67.4 & 42.2 & 58.1 & \multicolumn{1}{c|}{47.6} & 51.9 & 52.5 \\ \hline
    
\multicolumn{1}{l|}{EcoTTA~\cite{ecotta}} & \textit{3.46M} & \textit{251.2MB} & \textit{\textcolor{darkcerulean}{MetaNet}} & 44.1 & 69.6 & 35.3 & 58.2 & \multicolumn{1}{c|}{49.6} & 51.3 & 41.9 & 66.1 & 31.5 & 55.3 & \multicolumn{1}{c|}{46.2} & 48.2 & 49.7 \\ 
\multicolumn{1}{l|}{~~~~~~~~~~~~~~~~~~~~~~~~~~~~+ \textit{w/WAD}} & \textit{3.46M} & \textit{251.2MB} & \textit{\textcolor{darkcerulean}{MetaNet}} & 44.6 & 70.2 & 41.6 & 58.0 & \multicolumn{1}{c|}{49.9} & 52.9 & 41.1 & 65.6 & 27.0 & 53.2 & \multicolumn{1}{c|}{45.3} & 46.4 & 49.6 \\ \hline

\multicolumn{1}{l|}{\cellcolor{g}BECoTTA (Ours)-S} &
\cellcolor{g}\textit{0.09M} & 
\cellcolor{g}\textit{211.2MB} &
\cellcolor{g}\textit{\textcolor{darkcerulean}{MoDE}} & 
\cellcolor{g}42.9 &
\cellcolor{g}68.5 &
\cellcolor{g}35.0 &
\cellcolor{g}57.2 &
\multicolumn{1}{c|}{\cellcolor{g}47.8} &
\cellcolor{g}50.5 &
\cellcolor{g}43.0 &
\cellcolor{g}69.5 &
\cellcolor{g}35.1 &
\cellcolor{g}57.3 &
\multicolumn{1}{c|}{\cellcolor{g}48.8} &
\cellcolor{g}50.7 &
\cellcolor{g}50.6 \\

\multicolumn{1}{l|}{\cellcolor{g}~~~~~~~~~~~~~~~~~~~~~~~~~~~~+ \textit{w/WAD}} &
\cellcolor{g}\textit{0.12M} & 
\cellcolor{g}\textit{227.8MB} &
\cellcolor{g}\textit{\textcolor{darkcerulean}{MoDE}} & 
\cellcolor{g}44.1 &
\cellcolor{g}69.5 &
\cellcolor{g}40.1 &
\cellcolor{g}56.8 &
\multicolumn{1}{c|}{\cellcolor{g}49.1} &
\cellcolor{g}51.9 &
\cellcolor{g}44.0 &
\cellcolor{g}69.4 &
\cellcolor{g}40.1 &
\cellcolor{g}56.9 &
\multicolumn{1}{c|}{\cellcolor{g}49.1} &
\cellcolor{g}51.9 &
\cellcolor{g}51.9 \\ \hline

\multicolumn{1}{l|}{\cellcolor{gg}BECoTTA (Ours)-M} & 
\cellcolor{gg}\textit{0.63M} & 
\cellcolor{gg}\textit{221.3MB} &
\cellcolor{gg}\textit{\textcolor{darkcerulean}{MoDE}} & 
\cellcolor{gg}43.8 &
\cellcolor{gg}68.8 &
\cellcolor{gg}34.9 &
\cellcolor{gg}57.9 &
\multicolumn{1}{c|}{\cellcolor{gg}49.2} & 
\cellcolor{gg}50.9 & 
\cellcolor{gg}43.7 & 
\cellcolor{gg}68.8 & 
\cellcolor{gg}34.5 & 
\cellcolor{gg}57.9 & 
\multicolumn{1}{c|}{\cellcolor{gg}49.2} &
\cellcolor{gg}50.9 &
\cellcolor{gg}50.9 \\

\multicolumn{1}{l|}{\cellcolor{gg}~~~~~~~~~~~~~~~~~~~~~~~~~~~~+ \textit{w/WAD}} &
\cellcolor{gg}\textit{0.77M} &  
\cellcolor{gg}\textit{234.0MB} &
\cellcolor{gg}\textit{\textcolor{darkcerulean}{MoDE}} & 
\cellcolor{gg}45.6 & 
\cellcolor{gg}70.8 & 
\cellcolor{gg}42.6 & 
\cellcolor{gg}59.6 & 
\multicolumn{1}{c|}{\cellcolor{gg}\textbf{50.8}} & 
\cellcolor{gg}53.9 & 
\cellcolor{gg}45.6 & 
\cellcolor{gg}70.7 & 
\cellcolor{gg}42.5 & 
\cellcolor{gg}59.5 & 
\multicolumn{1}{c|}{\cellcolor{gg}\textbf{50.8}} & 
\cellcolor{gg}53.9 & 
\cellcolor{gg}53.9 \\ \hline

\multicolumn{1}{l|}{\cellcolor{ggg} BECoTTA (Ours)-L} &
\cellcolor{ggg} \textit{3.16M} & 
\cellcolor{ggg}\textit{240.7MB} &
\cellcolor{ggg}\textit{\textcolor{darkcerulean}{MoDE}} & 
\cellcolor{ggg}43.9 &
\cellcolor{ggg}69.1 &
\cellcolor{ggg}35.0 &
\cellcolor{ggg}58.3 &
\multicolumn{1}{c|}{\cellcolor{ggg}50.2} &
\cellcolor{ggg}51.3 &
\cellcolor{ggg}44.0 &
\cellcolor{ggg}69.1 &
\cellcolor{ggg}35.1 &
\cellcolor{ggg}58.3 &
\multicolumn{1}{c|}{\cellcolor{ggg}50.2} &
\cellcolor{ggg}51.3 &
\cellcolor{ggg}51.3 \\

\multicolumn{1}{l|}{\cellcolor{ggg}~~~~~~~~~~~~~~~~~~~~~~~~~~~~+ \textit{w/WAD}} &
\cellcolor{ggg} \textit{3.32M} & 
\cellcolor{ggg}\textit{300.0MB} &
\cellcolor{ggg}\textit{\textcolor{darkcerulean}{MoDE}} & 
\cellcolor{ggg}\textbf{45.7} &
\cellcolor{ggg}\textbf{71.4} &
\cellcolor{ggg}\textbf{43.7} &
\cellcolor{ggg}\textbf{59.6} &
\multicolumn{1}{c|}{\cellcolor{ggg}50.5} &
\cellcolor{ggg}\textbf{54.2} &
\cellcolor{ggg}\textbf{45.7} &
\cellcolor{ggg}\textbf{71.3} &
\cellcolor{ggg}\textbf{43.7} &
\cellcolor{ggg}\textbf{59.6} &
\multicolumn{1}{c|}{\cellcolor{ggg}50.6} &
\cellcolor{ggg}\textbf{54.2} &
\cellcolor{ggg}\textbf{54.2} \\
\bottomrule
\end{tabular}%
}
\label{ref:main2_v2}
\end{table*}


% \definecolor{airforceblue}{rgb}{0.36, 0.54, 0.66}
% \definecolor{ao(english)}{rgb}{0.0, 0.5, 0.0}
% \definecolor{azure(colorwheel)}{rgb}{0.0, 0.5, 1.0}
% \definecolor{crimson}{rgb}{0.86, 0.08, 0.24}
% \definecolor{darkcerulean}{rgb}{0.03, 0.27, 0.49}
% \definecolor{cobalt}{rgb}{0.0, 0.28, 0.67}
% \definecolor{rosegold}{rgb}{0.72, 0.43, 0.47}
% \definecolor{orange-red}{rgb}{1.0, 0.27, 0.0}
% \definecolor{mountainmeadow}{rgb}{0.19, 0.73, 0.56}
% \definecolor{malachite}{rgb}{0.04, 0.85, 0.32}
% \definecolor{darkblue}{rgb}{0.0, 0.0, 0.55}
% \definecolor{customblue}{rgb}{0.2, 0.35, 0.8}



% \begin{table*}[h]
% \centering
% \renewcommand{\arraystretch}{1.2}
% \caption{\textbf{Quantitative results of \textit{CDS-(ii) imbalanced weather \& area shifts} scenario.} We devised a novel scenario encompassing imbalanced weather and area shifts. We presented performance results for both \textit{w/o WAD} and \textit{w/ WAD} across the overall baselines. Given that our BECoTTA can take on different versions based on the number of experts and hidden dimensions, we reported both $M$ and $L$ versions, corresponding to variations in the number of parameters. \daeun{column split}}

% \setlength{\tabcolsep}{.2em}
% \resizebox{\linewidth}{!}{%
% \begin{tabular}{lc|cccccc|cccccc|c}
% \toprule
% \multicolumn{2}{c|}{Round} & \multicolumn{6}{c|}{\textbf{1}} & \multicolumn{6}{c|}{\textbf{10}} & \multirow{2}{*}{Total Mean} \\ \cline{1-14}

% \multicolumn{1}{c|}{Method} & Parameters & B-Clear & A-Fog & A-Night & A-Snow & \multicolumn{1}{c|}{B-Overcast} & Mean & \multicolumn{1}{l}{B-clear} & \multicolumn{1}{l}{A-Fog} & \multicolumn{1}{l}{A-Night} & \multicolumn{1}{l}{A-Snow} & \multicolumn{1}{l|}{B-Overcast} & \multicolumn{1}{l|}{Mean} &  \\ \hline \hline

% \multicolumn{1}{l|}{Source only} & - & 41.0 & 64.4 & 33.4 & 54.3 & \multicolumn{1}{c|}{46.3} & 47.9 & 41.0 & 64.4 & 33.4 & 54.3 & \multicolumn{1}{c|}{46.3} & 47.9 & 47.9 \\ 
% \multicolumn{1}{l|}{~~~~~~~~~~+ \textit{\textcolor{orange}{Full} updated w/WAD}} & - & 43.6 & 68.7 & 44.5 & 59.0 & \multicolumn{1}{c|}{48.7} & 52.9 & 43.6 & 68.7 & 44.5 & 59.0 & \multicolumn{1}{c|}{48.7} & 52.9 & 52.9 \\ \hline 

% \multicolumn{1}{l|}{CoTTA~\cite{cotta}} & \textit{54.72M} & 43.3 & 67.3 & 34.8 & 56.9 & \multicolumn{1}{c|}{48.8} & 50.2 & 43.3 & 67.3 & 34.8 & 56.9 & \multicolumn{1}{c|}{48.8} & 50.2 & 50.3 \\
% \multicolumn{1}{l|}{~~~~~~~~~~+ \textit{\textcolor{orange}{Full} updated w/WAD}} & \textit{54.72M} & 46.4 & 70.6 & 45.7 & 61.2 & \multicolumn{1}{c|}{51.3} & 55.0 & 46.1 & 70.5 & 45.6 & 61.1 & \multicolumn{1}{c|}{51.2} & 54.9 & 54.9 \\ \hline 

% \multicolumn{1}{l|}{TENT~\cite{tent}} & \textit{0.02M} & 41.1 & 64.9 & 33.2 & 54.3 & \multicolumn{1}{c|}{46.3} & 47.9 & 30.9 & 51.5 & 20.4 & 37.0 & \multicolumn{1}{c|}{33.0} & 34.6 & 42.7 \\

% \multicolumn{1}{l|}{~~~~~~~~~~+ \textit{\textcolor{orange}{Full} updated w/WAD}} & \textit{0.02M} & 43.7 & 68.5 & 44.6 & 59.0 & \multicolumn{1}{c|}{48.3} & 52.8 & 35.8 & 57.6 & 33.6 & 44.3 & \multicolumn{1}{c|}{38.8} & 42.0 & 48.4 \\ \hline 
    
% \multicolumn{1}{l|}{SAR~\cite{sar}} & \textit{0.02M} & 41.0 & 64.5 & 33.4 & 54.5 & \multicolumn{1}{c|}{46.6} & 48.0 & 41.3 & 64.3 & 31.6 & 54.2 & \multicolumn{1}{c|}{46.6} & 47.6 & 47.9 \\
% \multicolumn{1}{l|}{~~~~~~~~~~+ \textit{\textcolor{orange}{Full} updated w/WAD}} & \textit{0.02M} & 43.6 & 68.6 & 44.5 & 59.1 & \multicolumn{1}{c|}{48.7} & 52.9 & 43.4 & 67.4 & 42.2 & 58.1 & \multicolumn{1}{c|}{47.6} & 51.9 & 52.5 \\ \hline
    
% \multicolumn{1}{l|}{EcoTTA~\cite{ecotta}} & \textit{3.46M} & 44.1 & 69.6 & 35.3 & 58.2 & \multicolumn{1}{c|}{49.6} & 51.3 & 41.9 & 66.1 & 31.5 & 55.3 & \multicolumn{1}{c|}{46.2} & 48.2 & 49.7 \\ 
% \multicolumn{1}{l|}{~~~~~~~~~~+ \textit{\textcolor{blue}{MetaNet} updated w/WAD}} & \textit{3.46M} & 44.6 & 70.2 & 41.6 & 58.0 & \multicolumn{1}{c|}{49.9} & 52.9 & 41.1 & 65.6 & 27.0 & 53.2 & \multicolumn{1}{c|}{45.3} & 46.4 & 49.6 \\ \hline

% \multicolumn{1}{l|}{\cellcolor{g}BECoTTA (Ours)-S} &
% \cellcolor{g}\textit{0.09M} &
% \cellcolor{g}42.9 &
% \cellcolor{g}68.5 &
% \cellcolor{g}35.0 &
% \cellcolor{g}57.2 &
% \multicolumn{1}{c|}{\cellcolor{g}47.8} &
% \cellcolor{g}50.5 &
% \cellcolor{g} &
% \cellcolor{g} &
% \cellcolor{g} &
% \cellcolor{g} &
% \multicolumn{1}{c|}{\cellcolor{g}} &
% \cellcolor{g} &
% \cellcolor{g} \\

% \multicolumn{1}{l|}{\cellcolor{g}~~~~~~~~~~+ \textit{\textcolor{blue}{MoDE} updated w/WAD}} &
% \cellcolor{g}\textit{0.12M} &
% \cellcolor{g}44.1 &
% \cellcolor{g}69.5 &
% \cellcolor{g}40.1 &
% \cellcolor{g}56.8 &
% \multicolumn{1}{c|}{\cellcolor{g}49.1} &
% \cellcolor{g}51.9 &
% \cellcolor{g} &
% \cellcolor{g} &
% \cellcolor{g} &
% \cellcolor{g} &
% \multicolumn{1}{c|}{\cellcolor{g}} &
% \cellcolor{g} &
% \cellcolor{g} \\ \hline

% \multicolumn{1}{l|}{\cellcolor{gg}BECoTTA (Ours)-M} & 
% \cellcolor{gg}\textit{0.63M} &
% \cellcolor{gg}43.8 &
% \cellcolor{gg}68.8 &
% \cellcolor{gg}34.9 &
% \cellcolor{gg}57.9 &
% \multicolumn{1}{c|}{\cellcolor{gg}49.2} & 
% \cellcolor{gg}50.9 & 
% \cellcolor{gg}43.7 & 
% \cellcolor{gg}68.8 & 
% \cellcolor{gg}34.5 & 
% \cellcolor{gg}57.9 & 
% \multicolumn{1}{c|}{\cellcolor{gg}49.2} &
% \cellcolor{gg}50.9 &
% \cellcolor{gg}50.9 \\
% \multicolumn{1}{l|}{\cellcolor{gg}~~~~~~~~~~+ \textit{\textcolor{blue}{MoDE} updated w/WAD}} &
% \cellcolor{gg}\textit{0.77M} & 
% \cellcolor{gg}45.6 & 
% \cellcolor{gg}70.8 & 
% \cellcolor{gg}42.6 & 
% \cellcolor{gg}59.7 & 
% \multicolumn{1}{c|}{\cellcolor{gg}50.8} & 
% \cellcolor{gg}53.9 & 
% \cellcolor{gg}45.6 & 
% \cellcolor{gg}70.7 & 
% \cellcolor{gg}42.5 & 
% \cellcolor{gg}59.5 & 
% \multicolumn{1}{c|}{\cellcolor{gg}50.8} & 
% \cellcolor{gg}53.9 & 
% \cellcolor{gg}53.9 \\ \hline

% \multicolumn{1}{l|}{\cellcolor{ggg} BECoTTA (Ours)-L} &
% \cellcolor{ggg} \textit{3.16M} &
% \cellcolor{ggg}43.9 &
% \cellcolor{ggg}69.1 &
% \cellcolor{ggg} &
% \cellcolor{ggg} &
% \multicolumn{1}{c|}{\cellcolor{ggg}} &
% \cellcolor{ggg} &
% \cellcolor{ggg} &
% \cellcolor{ggg} &
% \cellcolor{ggg} &
% \cellcolor{ggg} &
% \multicolumn{1}{c|}{\cellcolor{ggg}} &
% \cellcolor{ggg} &
% \cellcolor{ggg} \\

% \multicolumn{1}{l|}{\cellcolor{ggg}~~~~~~~~~~+ \textit{\textcolor{blue}{MoDE} updated w/WAD}} &
% \cellcolor{ggg} \textit{3.32M} &
% \cellcolor{ggg}45.7 &
% \cellcolor{ggg}70.4 &
% \cellcolor{ggg}43.6 &
% \cellcolor{ggg} &
% \multicolumn{1}{c|}{\cellcolor{ggg}} &
% \cellcolor{ggg} &
% \cellcolor{ggg} &
% \cellcolor{ggg} &
% \cellcolor{ggg} &
% \cellcolor{ggg} &
% \multicolumn{1}{c|}{\cellcolor{ggg}} &
% \cellcolor{ggg} &
% \cellcolor{ggg} \\
% \bottomrule
% \end{tabular}%
% }
% \label{ref:main2_v2}
% \end{table*}



